The SDSS Quasar Survey: Quasar Luminosity Function from Data Release Three

We determine the number counts and z=0-5 luminosity function for a well-defined, homogeneous sample of quasars from the Sloan Digital Sky Survey (SDSS). We conservatively define the most uniform statistical sample possible, consisting of 15,343 quasars within an effective area of 1622 deg^2 that was derived from a parent sample of 46,420 spectroscopically confirmed broad-line quasars in the 5282 deg^2 of imaging data from SDSS Data Release Three. The sample extends from i=15 to i=19.1 at z<3 and to i=20.2 for z>3. The number counts and luminosity function agree well with the results of the 2dF QSO Survey, but the SDSS data probe to much higher redshifts than does the 2dF sample. The number density of luminous quasars peaks between redshifts 2 and 3, although uncertainties in the selection function in this range do not allow us to determine the peak redshift more precisely. Our best fit model has a flatter bright end slope at high redshift than at low redshift. For z<2.4 the data are best fit by a redshift-independent slope of beta = -3.1 (Phi(L) propto L^beta). Above z=2.4 the slope flattens with redshift to beta=-2.37 at z=5. This slope change, which is significant at a >5-sigma level, must be accounted for in models of the evolution of accretion onto supermassive black holes.

==> tab2.tex <==
15.475 & $0.00\pm0.00$  & $0.00\pm0.00$ &    2 & $0.00\pm0.00$  & $0.00\pm0.00$ &    1 \\
15.725 & $0.00\pm0.00$  & $0.00\pm0.00$ &    3 & $0.00\pm0.00$  & $0.00\pm0.00$ &    3 \\
15.975 & $0.00\pm0.00$  & $0.01\pm0.00$ &    4 & $0.00\pm0.00$  & $0.00\pm0.00$ &    2 \\
16.225 & $0.01\pm0.00$  & $0.01\pm0.00$ &   11 & $0.01\pm0.00$  & $0.01\pm0.00$ &   10 \\
16.475 & $0.01\pm0.00$  & $0.02\pm0.00$ &   10 & $0.01\pm0.00$  & $0.02\pm0.00$ &   12 \\
16.725 & $0.02\pm0.00$  & $0.04\pm0.00$ &   32 & $0.01\pm0.00$  & $0.03\pm0.00$ &   23 \\
16.975 & $0.06\pm0.01$  & $0.10\pm0.01$ &   85 & $0.04\pm0.01$  & $0.08\pm0.01$ &   67 \\
17.225 & $0.08\pm0.01$  & $0.17\pm0.01$ &  117 & $0.07\pm0.01$  & $0.15\pm0.01$ &  107 \\
17.475 & $0.12\pm0.01$  & $0.29\pm0.01$ &  190 & $0.11\pm0.01$  & $0.26\pm0.01$ &  174 \\
17.725 & $0.23\pm0.01$  & $0.53\pm0.01$ &  357 & $0.21\pm0.01$  & $0.47\pm0.01$ &  327 \\
17.975 & $0.31\pm0.01$  & $0.83\pm0.01$ &  472 & $0.33\pm0.01$  & $0.80\pm0.01$ &  511 \\
18.225 & $0.56\pm0.02$  & $1.40\pm0.02$ &  868 & $0.55\pm0.02$  & $1.35\pm0.02$ &  849 \\
18.475 & $0.78\pm0.02$  & $2.18\pm0.02$ & 1202 & $0.82\pm0.02$  & $2.17\pm0.02$ & 1257 \\
18.725 & $1.19\pm0.03$  & $3.37\pm0.03$ & 1839 & $1.25\pm0.03$  & $3.42\pm0.03$ & 1923 \\
18.975 & $1.70\pm0.03$  & $5.07\pm0.03$ & 2620 & $1.86\pm0.04$  & $5.28\pm0.03$ & 2870 \\
19.225 & $1.61\pm0.03$  & $6.68\pm0.03$ & 2484 & $2.62\pm0.04$  & $7.90\pm0.04$ & 4028 \\
19.475 & $0.56\pm0.02$  & $7.24\pm0.02$ &  855 & \ldots  & \ldots &  900 \\
19.725 & $0.13\pm0.01$  & $7.37\pm0.01$ &  206 & \ldots  & \ldots &  216 \\
19.975 & $0.03\pm0.01$  & $7.41\pm0.00$ &   53 & \ldots  & \ldots &   55 \\
20.225 & $0.01\pm0.00$  & $7.42\pm0.00$ &   19 & \ldots  & \ldots &   20 \\


==> tab3.tex <==
17.075 & $0.00\pm0.00$  & $0.00\pm0.00$ &    1 &  1.1 \\
17.325 & $0.00\pm0.00$  & $0.00\pm0.00$ &    4 &  4.5 \\
17.575 & $0.01\pm0.00$  & $0.01\pm0.00$ &   12 & 14.2 \\
17.825 & $0.01\pm0.00$  & $0.02\pm0.00$ &   12 & 14.2 \\
18.075 & $0.02\pm0.00$  & $0.04\pm0.00$ &   26 & 29.7 \\
18.325 & $0.03\pm0.01$  & $0.07\pm0.00$ &   47 & 55.8 \\
18.575 & $0.05\pm0.01$  & $0.13\pm0.01$ &   72 & 83.8 \\
18.825 & $0.08\pm0.01$  & $0.20\pm0.01$ &  106 & 124.7 \\
19.075 & $0.12\pm0.01$  & $0.33\pm0.01$ &  162 & 197.5 \\
19.325 & $0.17\pm0.01$  & $0.49\pm0.01$ &  206 & 268.4 \\
19.575 & $0.22\pm0.01$  & $0.71\pm0.01$ &  275 & 360.2 \\
19.825 & $0.28\pm0.02$  & $0.99\pm0.01$ &  322 & 455.4 \\
20.075 & $0.38\pm0.02$  & $1.37\pm0.02$ &  410 & 617.5 \\


==> tab4.tex <==
0.00 & $0.596$ \\
0.01 & $0.587$ \\
0.02 & $0.569$ \\
0.03 & $0.531$ \\
0.04 & $0.462$ \\
0.05 & $0.372$ \\
0.06 & $0.268$ \\
0.07 & $0.203$ \\
0.08 & $0.170$ \\
0.09 & $0.157$ \\
0.10 & $0.156$ \\
0.11 & $0.155$ \\
0.12 & $0.154$ \\
0.13 & $0.160$ \\
0.14 & $0.167$ \\
0.15 & $0.184$ \\
0.16 & $0.241$ \\
0.17 & $0.208$ \\
0.18 & $0.193$ \\
0.19 & $0.192$ \\
0.20 & $0.197$ \\
0.21 & $0.201$ \\
0.22 & $0.208$ \\
0.23 & $0.224$ \\
0.24 & $0.263$ \\
0.25 & $0.337$ \\
0.26 & $0.406$ \\
0.27 & $0.447$ \\
0.28 & $0.462$ \\
0.29 & $0.467$ \\
0.30 & $0.465$ \\
0.31 & $0.457$ \\
0.32 & $0.450$ \\
0.33 & $0.441$ \\
0.34 & $0.433$ \\
0.35 & $0.424$ \\
0.36 & $0.416$ \\
0.37 & $0.405$ \\
0.38 & $0.391$ \\
0.39 & $0.374$ \\
0.40 & $0.355$ \\
0.41 & $0.334$ \\
0.42 & $0.312$ \\
0.43 & $0.291$ \\
0.44 & $0.276$ \\
0.45 & $0.264$ \\
0.46 & $0.257$ \\
0.47 & $0.252$ \\
0.48 & $0.247$ \\
0.49 & $0.240$ \\
0.50 & $0.235$ \\
0.51 & $0.229$ \\
0.52 & $0.232$ \\
0.53 & $0.224$ \\
0.54 & $0.220$ \\
0.55 & $0.219$ \\
0.56 & $0.224$ \\
0.57 & $0.225$ \\
0.58 & $0.214$ \\
0.59 & $0.205$ \\
0.60 & $0.197$ \\
0.61 & $0.191$ \\
0.62 & $0.189$ \\
0.63 & $0.191$ \\
0.64 & $0.196$ \\
0.65 & $0.202$ \\
0.66 & $0.209$ \\
0.67 & $0.216$ \\
0.68 & $0.226$ \\
0.69 & $0.236$ \\
0.70 & $0.243$ \\
0.71 & $0.247$ \\
0.72 & $0.246$ \\
0.73 & $0.244$ \\
0.74 & $0.243$ \\
0.75 & $0.242$ \\
0.76 & $0.238$ \\
0.77 & $0.230$ \\
0.78 & $0.223$ \\
0.79 & $0.218$ \\
0.80 & $0.212$ \\
0.81 & $0.207$ \\
0.82 & $0.202$ \\
0.83 & $0.195$ \\
0.84 & $0.189$ \\
0.85 & $0.182$ \\
0.86 & $0.175$ \\
0.87 & $0.167$ \\
0.88 & $0.161$ \\
0.89 & $0.156$ \\
0.90 & $0.151$ \\
0.91 & $0.145$ \\
0.92 & $0.139$ \\
0.93 & $0.130$ \\
0.94 & $0.120$ \\
0.95 & $0.111$ \\
0.96 & $0.102$ \\
0.97 & $0.093$ \\
0.98 & $0.082$ \\
0.99 & $0.071$ \\
1.00 & $0.061$ \\
1.01 & $0.051$ \\
1.02 & $0.041$ \\
1.03 & $0.031$ \\
1.04 & $0.021$ \\
1.05 & $0.010$ \\
1.06 & $0.001$ \\
1.07 & $-0.009$ \\
1.08 & $-0.018$ \\
1.09 & $-0.025$ \\
1.10 & $-0.033$ \\
1.11 & $-0.041$ \\
1.12 & $-0.048$ \\
1.13 & $-0.056$ \\
1.14 & $-0.065$ \\
1.15 & $-0.072$ \\
1.16 & $-0.080$ \\
1.17 & $-0.087$ \\
1.18 & $-0.092$ \\
1.19 & $-0.098$ \\
1.20 & $-0.104$ \\
1.21 & $-0.108$ \\
1.22 & $-0.112$ \\
1.23 & $-0.117$ \\
1.24 & $-0.121$ \\
1.25 & $-0.124$ \\
1.26 & $-0.128$ \\
1.27 & $-0.131$ \\
1.28 & $-0.133$ \\
1.29 & $-0.136$ \\
1.30 & $-0.140$ \\
1.31 & $-0.143$ \\
1.32 & $-0.147$ \\
1.33 & $-0.151$ \\
1.34 & $-0.155$ \\
1.35 & $-0.158$ \\
1.36 & $-0.162$ \\
1.37 & $-0.166$ \\
1.38 & $-0.168$ \\
1.39 & $-0.172$ \\
1.40 & $-0.176$ \\
1.41 & $-0.181$ \\
1.42 & $-0.187$ \\
1.43 & $-0.193$ \\
1.44 & $-0.201$ \\
1.45 & $-0.209$ \\
1.46 & $-0.218$ \\
1.47 & $-0.228$ \\
1.48 & $-0.236$ \\
1.49 & $-0.245$ \\
1.50 & $-0.252$ \\
1.51 & $-0.258$ \\
1.52 & $-0.261$ \\
1.53 & $-0.265$ \\
1.54 & $-0.267$ \\
1.55 & $-0.268$ \\
1.56 & $-0.268$ \\
1.57 & $-0.268$ \\
1.58 & $-0.268$ \\
1.59 & $-0.268$ \\
1.60 & $-0.268$ \\
1.61 & $-0.269$ \\
1.62 & $-0.270$ \\
1.63 & $-0.270$ \\
1.64 & $-0.270$ \\
1.65 & $-0.271$ \\
1.66 & $-0.272$ \\
1.67 & $-0.272$ \\
1.68 & $-0.273$ \\
1.69 & $-0.274$ \\
1.70 & $-0.274$ \\
1.71 & $-0.271$ \\
1.72 & $-0.271$ \\
1.73 & $-0.273$ \\
1.74 & $-0.277$ \\
1.75 & $-0.279$ \\
1.76 & $-0.281$ \\
1.77 & $-0.282$ \\
1.78 & $-0.283$ \\
1.79 & $-0.283$ \\
1.80 & $-0.284$ \\
1.81 & $-0.285$ \\
1.82 & $-0.286$ \\
1.83 & $-0.286$ \\
1.84 & $-0.287$ \\
1.85 & $-0.287$ \\
1.86 & $-0.287$ \\
1.87 & $-0.286$ \\
1.88 & $-0.285$ \\
1.89 & $-0.283$ \\
1.90 & $-0.280$ \\
1.91 & $-0.275$ \\
1.92 & $-0.271$ \\
1.93 & $-0.266$ \\
1.94 & $-0.262$ \\
1.95 & $-0.257$ \\
1.96 & $-0.253$ \\
1.97 & $-0.250$ \\
1.98 & $-0.248$ \\
1.99 & $-0.245$ \\
2.00 & $-0.244$ \\
2.01 & $-0.243$ \\
2.02 & $-0.242$ \\
2.03 & $-0.241$ \\
2.04 & $-0.239$ \\
2.05 & $-0.238$ \\
2.06 & $-0.238$ \\
2.07 & $-0.237$ \\
2.08 & $-0.235$ \\
2.09 & $-0.234$ \\
2.10 & $-0.233$ \\
2.11 & $-0.231$ \\
2.12 & $-0.230$ \\
2.13 & $-0.227$ \\
2.14 & $-0.226$ \\
2.15 & $-0.224$ \\
2.16 & $-0.223$ \\
2.17 & $-0.221$ \\
2.18 & $-0.220$ \\
2.19 & $-0.219$ \\
2.20 & $-0.218$ \\
2.21 & $-0.216$ \\
2.22 & $-0.214$ \\
2.23 & $-0.213$ \\
2.24 & $-0.212$ \\
2.25 & $-0.211$ \\
2.26 & $-0.208$ \\
2.27 & $-0.207$ \\
2.28 & $-0.207$ \\
2.29 & $-0.207$ \\
2.30 & $-0.206$ \\
2.31 & $-0.205$ \\
2.32 & $-0.205$ \\
2.33 & $-0.205$ \\
2.34 & $-0.205$ \\
2.35 & $-0.206$ \\
2.36 & $-0.205$ \\
2.37 & $-0.204$ \\
2.38 & $-0.204$ \\
2.39 & $-0.204$ \\
2.40 & $-0.204$ \\
2.41 & $-0.203$ \\
2.42 & $-0.203$ \\
2.43 & $-0.203$ \\
2.44 & $-0.203$ \\
2.45 & $-0.203$ \\
2.46 & $-0.202$ \\
2.47 & $-0.203$ \\
2.48 & $-0.203$ \\
2.49 & $-0.203$ \\
2.50 & $-0.204$ \\
2.51 & $-0.204$ \\
2.52 & $-0.205$ \\
2.53 & $-0.207$ \\
2.54 & $-0.209$ \\
2.55 & $-0.211$ \\
2.56 & $-0.213$ \\
2.57 & $-0.216$ \\
2.58 & $-0.221$ \\
2.59 & $-0.225$ \\
2.60 & $-0.230$ \\
2.61 & $-0.235$ \\
2.62 & $-0.241$ \\
2.63 & $-0.247$ \\
2.64 & $-0.253$ \\
2.65 & $-0.260$ \\
2.66 & $-0.265$ \\
2.67 & $-0.270$ \\
2.68 & $-0.276$ \\
2.69 & $-0.281$ \\
2.70 & $-0.285$ \\
2.71 & $-0.289$ \\
2.72 & $-0.293$ \\
2.73 & $-0.296$ \\
2.74 & $-0.299$ \\
2.75 & $-0.302$ \\
2.76 & $-0.304$ \\
2.77 & $-0.305$ \\
2.78 & $-0.307$ \\
2.79 & $-0.308$ \\
2.80 & $-0.310$ \\
2.81 & $-0.311$ \\
2.82 & $-0.312$ \\
2.83 & $-0.313$ \\
2.84 & $-0.314$ \\
2.85 & $-0.315$ \\
2.86 & $-0.316$ \\
2.87 & $-0.317$ \\
2.88 & $-0.317$ \\
2.89 & $-0.317$ \\
2.90 & $-0.318$ \\
2.91 & $-0.318$ \\
2.92 & $-0.318$ \\
2.93 & $-0.317$ \\
2.94 & $-0.317$ \\
2.95 & $-0.317$ \\
2.96 & $-0.316$ \\
2.97 & $-0.315$ \\
2.98 & $-0.314$ \\
2.99 & $-0.312$ \\
3.00 & $-0.312$ \\
3.01 & $-0.313$ \\
3.02 & $-0.314$ \\
3.03 & $-0.316$ \\
3.04 & $-0.318$ \\
3.05 & $-0.318$ \\
3.06 & $-0.319$ \\
3.07 & $-0.320$ \\
3.08 & $-0.321$ \\
3.09 & $-0.322$ \\
3.10 & $-0.323$ \\
3.11 & $-0.323$ \\
3.12 & $-0.324$ \\
3.13 & $-0.325$ \\
3.14 & $-0.327$ \\
3.15 & $-0.328$ \\
3.16 & $-0.330$ \\
3.17 & $-0.330$ \\
3.18 & $-0.331$ \\
3.19 & $-0.333$ \\
3.20 & $-0.334$ \\
3.21 & $-0.335$ \\
3.22 & $-0.336$ \\
3.23 & $-0.336$ \\
3.24 & $-0.336$ \\
3.25 & $-0.336$ \\
3.26 & $-0.336$ \\
3.27 & $-0.336$ \\
3.28 & $-0.335$ \\
3.29 & $-0.333$ \\
3.30 & $-0.332$ \\
3.31 & $-0.330$ \\
3.32 & $-0.329$ \\
3.33 & $-0.328$ \\
3.34 & $-0.328$ \\
3.35 & $-0.327$ \\
3.36 & $-0.327$ \\
3.37 & $-0.329$ \\
3.38 & $-0.331$ \\
3.39 & $-0.333$ \\
3.40 & $-0.337$ \\
3.41 & $-0.339$ \\
3.42 & $-0.343$ \\
3.43 & $-0.348$ \\
3.44 & $-0.353$ \\
3.45 & $-0.359$ \\
3.46 & $-0.365$ \\
3.47 & $-0.371$ \\
3.48 & $-0.376$ \\
3.49 & $-0.383$ \\
3.50 & $-0.388$ \\
3.51 & $-0.394$ \\
3.52 & $-0.398$ \\
3.53 & $-0.403$ \\
3.54 & $-0.405$ \\
3.55 & $-0.408$ \\
3.56 & $-0.411$ \\
3.57 & $-0.413$ \\
3.58 & $-0.414$ \\
3.59 & $-0.416$ \\
3.60 & $-0.417$ \\
3.61 & $-0.416$ \\
3.62 & $-0.417$ \\
3.63 & $-0.416$ \\
3.64 & $-0.416$ \\
3.65 & $-0.415$ \\
3.66 & $-0.415$ \\
3.67 & $-0.414$ \\
3.68 & $-0.412$ \\
3.69 & $-0.412$ \\
3.70 & $-0.411$ \\
3.71 & $-0.410$ \\
3.72 & $-0.409$ \\
3.73 & $-0.409$ \\
3.74 & $-0.407$ \\
3.75 & $-0.406$ \\
3.76 & $-0.405$ \\
3.77 & $-0.404$ \\
3.78 & $-0.404$ \\
3.79 & $-0.403$ \\
3.80 & $-0.402$ \\
3.81 & $-0.401$ \\
3.82 & $-0.400$ \\
3.83 & $-0.399$ \\
3.84 & $-0.399$ \\
3.85 & $-0.398$ \\
3.86 & $-0.397$ \\
3.87 & $-0.397$ \\
3.88 & $-0.394$ \\
3.89 & $-0.393$ \\
3.90 & $-0.391$ \\
3.91 & $-0.389$ \\
3.92 & $-0.388$ \\
3.93 & $-0.388$ \\
3.94 & $-0.390$ \\
3.95 & $-0.390$ \\
3.96 & $-0.393$ \\
3.97 & $-0.395$ \\
3.98 & $-0.396$ \\
3.99 & $-0.398$ \\
4.00 & $-0.399$ \\
4.01 & $-0.399$ \\
4.02 & $-0.399$ \\
4.03 & $-0.399$ \\
4.04 & $-0.399$ \\
4.05 & $-0.398$ \\
4.06 & $-0.398$ \\
4.07 & $-0.397$ \\
4.08 & $-0.396$ \\
4.09 & $-0.396$ \\
4.10 & $-0.394$ \\
4.11 & $-0.393$ \\
4.12 & $-0.392$ \\
4.13 & $-0.391$ \\
4.14 & $-0.390$ \\
4.15 & $-0.389$ \\
4.16 & $-0.388$ \\
4.17 & $-0.386$ \\
4.18 & $-0.385$ \\
4.19 & $-0.384$ \\
4.20 & $-0.383$ \\
4.21 & $-0.381$ \\
4.22 & $-0.380$ \\
4.23 & $-0.378$ \\
4.24 & $-0.375$ \\
4.25 & $-0.372$ \\
4.26 & $-0.369$ \\
4.27 & $-0.365$ \\
4.28 & $-0.361$ \\
4.29 & $-0.357$ \\
4.30 & $-0.353$ \\
4.31 & $-0.349$ \\
4.32 & $-0.344$ \\
4.33 & $-0.340$ \\
4.34 & $-0.337$ \\
4.35 & $-0.334$ \\
4.36 & $-0.331$ \\
4.37 & $-0.329$ \\
4.38 & $-0.327$ \\
4.39 & $-0.325$ \\
4.40 & $-0.323$ \\
4.41 & $-0.323$ \\
4.42 & $-0.322$ \\
4.43 & $-0.323$ \\
4.44 & $-0.324$ \\
4.45 & $-0.327$ \\
4.46 & $-0.330$ \\
4.47 & $-0.334$ \\
4.48 & $-0.337$ \\
4.49 & $-0.343$ \\
4.50 & $-0.348$ \\
4.51 & $-0.355$ \\
4.52 & $-0.362$ \\
4.53 & $-0.369$ \\
4.54 & $-0.377$ \\
4.55 & $-0.385$ \\
4.56 & $-0.393$ \\
4.57 & $-0.403$ \\
4.58 & $-0.413$ \\
4.59 & $-0.423$ \\
4.60 & $-0.434$ \\
4.61 & $-0.444$ \\
4.62 & $-0.455$ \\
4.63 & $-0.466$ \\
4.64 & $-0.475$ \\
4.65 & $-0.486$ \\
4.66 & $-0.496$ \\
4.67 & $-0.506$ \\
4.68 & $-0.515$ \\
4.69 & $-0.525$ \\
4.70 & $-0.534$ \\
4.71 & $-0.542$ \\
4.72 & $-0.549$ \\
4.73 & $-0.556$ \\
4.74 & $-0.562$ \\
4.75 & $-0.567$ \\
4.76 & $-0.571$ \\
4.77 & $-0.574$ \\
4.78 & $-0.576$ \\
4.79 & $-0.577$ \\
4.80 & $-0.577$ \\
4.81 & $-0.577$ \\
4.82 & $-0.575$ \\
4.83 & $-0.574$ \\
4.84 & $-0.572$ \\
4.85 & $-0.570$ \\
4.86 & $-0.567$ \\
4.87 & $-0.564$ \\
4.88 & $-0.560$ \\
4.89 & $-0.556$ \\
4.90 & $-0.552$ \\
4.91 & $-0.548$ \\
4.92 & $-0.544$ \\
4.93 & $-0.540$ \\
4.94 & $-0.536$ \\
4.95 & $-0.532$ \\
4.96 & $-0.528$ \\
4.97 & $-0.522$ \\
4.98 & $-0.518$ \\
4.99 & $-0.513$ \\
5.00 & $-0.509$ \\
5.01 & $-0.504$ \\
5.02 & $-0.500$ \\
5.03 & $-0.495$ \\
5.04 & $-0.490$ \\
5.05 & $-0.485$ \\
5.06 & $-0.480$ \\
5.07 & $-0.475$ \\
5.08 & $-0.470$ \\
5.09 & $-0.464$ \\
5.10 & $-0.458$ \\
5.11 & $-0.451$ \\
5.12 & $-0.445$ \\
5.13 & $-0.438$ \\
5.14 & $-0.431$ \\
5.15 & $-0.425$ \\
5.16 & $-0.419$ \\
5.17 & $-0.414$ \\
5.18 & $-0.409$ \\
5.19 & $-0.404$ \\
5.20 & $-0.398$ \\
5.21 & $-0.392$ \\
5.22 & $-0.385$ \\
5.23 & $-0.376$ \\
5.24 & $-0.367$ \\
5.25 & $-0.359$ \\
5.26 & $-0.352$ \\
5.27 & $-0.346$ \\
5.28 & $-0.343$ \\
5.29 & $-0.341$ \\
5.30 & $-0.340$ \\
5.31 & $-0.340$ \\
5.32 & $-0.338$ \\
5.33 & $-0.336$ \\
5.34 & $-0.334$ \\
5.35 & $-0.331$ \\
5.36 & $-0.328$ \\
5.37 & $-0.324$ \\
5.38 & $-0.320$ \\
5.39 & $-0.316$ \\
5.40 & $-0.312$ \\
5.41 & $-0.309$ \\
5.42 & $-0.303$ \\
5.43 & $-0.299$ \\
5.44 & $-0.295$ \\
5.45 & $-0.290$ \\
5.46 & $-0.285$ \\
5.47 & $-0.280$ \\
5.48 & $-0.275$ \\
5.49 & $-0.269$ \\


==> tab6.tex <==
0.49 & $-26.25$ & $-7.74$ & 5.48 & 1 & 0.59 & 11 & 11.6 \\
0.49 & $-25.95$ & $-7.46$ & 7.55 & 1 & 0.58 & 21 & 22.2 \\
0.49 & $-25.65$ & $-7.26$ & 9.47 & 1 & 0.58 & 33 & 34.8 \\
0.49 & $-25.35$ & $-7.07$ & 11.90 & 1 & 0.55 & 52 & 54.9 \\
0.49 & $-25.05$ & $-6.81$ & 16.01 & 1 & 0.56 & 94 & 99.3 \\
0.49 & $-24.75$ & $-6.59$ & 20.52 & 1 & 0.58 & 154 & 163.0 \\
0.49 & $-24.45$ & $-6.42$ & 24.94 & 1 & 0.57 & 228 & 241.0 \\
0.49 & $-24.15$ & $-6.23$ & 35.98 & 0 & 0.54 & 337 & 358.2 \\
0.49 & $-23.85$ & $-6.08$ & 43.96 & 0 & 0.51 & 358 & 377.2 \\
0.49 & $-23.55$ & $-5.97$ & 75.48 & 0 & 0.45 & 311 & 331.3 \\
0.49 & $-23.25$ & $-5.81$ & 102.81 & 0 & 0.41 & 290 & 307.2 \\
0.49 & $-22.95$ & $-6.35$ & 174.24 & 0 & 0.41 & 39 & 46.9 \\
0.87 & $-27.45$ & $-8.39$ & 1.81 & 1 & 0.95 & 5 & 5.3 \\
0.87 & $-27.15$ & $-7.81$ & 3.53 & 1 & 0.95 & 19 & 20.0 \\
0.87 & $-26.85$ & $-7.63$ & 4.36 & 1 & 0.95 & 29 & 30.5 \\
0.87 & $-26.55$ & $-7.29$ & 6.48 & 1 & 0.94 & 64 & 67.4 \\
0.87 & $-26.25$ & $-6.96$ & 9.38 & 1 & 0.91 & 134 & 141.2 \\
0.87 & $-25.95$ & $-6.84$ & 10.84 & 1 & 0.92 & 179 & 188.5 \\
0.87 & $-25.65$ & $-6.62$ & 13.87 & 1 & 0.92 & 293 & 308.6 \\
0.87 & $-25.35$ & $-6.42$ & 17.57 & 1 & 0.93 & 470 & 495.1 \\
0.87 & $-25.05$ & $-6.30$ & 24.49 & 0 & 0.89 & 492 & 520.0 \\
0.87 & $-24.75$ & $-6.23$ & 51.36 & 0 & 0.78 & 284 & 307.6 \\
0.87 & $-24.45$ & $-6.13$ & 100.79 & 0 & 0.73 & 122 & 133.7 \\
0.87 & $-24.15$ & $-5.86$ & 1446.59 & 0 & 0.74 & 9 & 13.8 \\
1.25 & $-28.05$ & $-8.15$ & 2.06 & 1 & 1.31 & 12 & 12.6 \\
1.25 & $-27.75$ & $-7.86$ & 2.85 & 1 & 1.32 & 23 & 24.2 \\
1.25 & $-27.45$ & $-7.76$ & 3.20 & 1 & 1.27 & 29 & 30.5 \\
1.25 & $-27.15$ & $-7.36$ & 5.07 & 1 & 1.30 & 73 & 76.8 \\
1.25 & $-26.85$ & $-7.08$ & 7.00 & 1 & 1.30 & 139 & 146.3 \\
1.25 & $-26.55$ & $-6.83$ & 9.37 & 1 & 1.29 & 249 & 262.1 \\
1.25 & $-26.25$ & $-6.58$ & 12.44 & 1 & 1.29 & 439 & 462.1 \\
1.25 & $-25.95$ & $-6.33$ & 16.62 & 1 & 1.28 & 783 & 824.2 \\
1.25 & $-25.65$ & $-6.24$ & 22.56 & 0 & 1.23 & 733 & 773.5 \\
1.25 & $-25.35$ & $-6.12$ & 48.01 & 0 & 1.13 & 360 & 382.8 \\
1.25 & $-25.05$ & $-5.74$ & 1332.39 & 0 & 1.09 & 12 & 14.6 \\
1.63 & $-28.65$ & $-8.25$ & 1.70 & 1 & 1.66 & 11 & 11.6 \\
1.63 & $-28.35$ & $-8.08$ & 2.06 & 1 & 1.67 & 16 & 16.8 \\
1.63 & $-28.05$ & $-7.78$ & 2.91 & 1 & 1.68 & 32 & 33.7 \\
1.63 & $-27.75$ & $-7.39$ & 4.57 & 1 & 1.66 & 79 & 83.2 \\
1.63 & $-27.45$ & $-7.12$ & 6.23 & 1 & 1.67 & 147 & 154.7 \\
1.63 & $-27.15$ & $-6.86$ & 8.43 & 1 & 1.66 & 269 & 283.2 \\
1.63 & $-26.85$ & $-6.63$ & 10.94 & 1 & 1.65 & 453 & 476.8 \\
1.63 & $-26.55$ & $-6.40$ & 14.35 & 1 & 1.66 & 779 & 820.0 \\
1.63 & $-26.25$ & $-6.26$ & 19.09 & 0 & 1.62 & 892 & 940.9 \\
1.63 & $-25.95$ & $-6.14$ & 38.86 & 0 & 1.52 & 477 & 506.0 \\
2.01 & $-28.95$ & $-8.41$ & 1.37 & 1 & 1.99 & 8 & 8.4 \\
2.01 & $-28.65$ & $-7.94$ & 2.37 & 1 & 2.02 & 24 & 25.3 \\
2.01 & $-28.35$ & $-7.75$ & 2.94 & 1 & 2.02 & 37 & 39.0 \\
2.01 & $-28.05$ & $-7.37$ & 4.53 & 1 & 2.01 & 88 & 92.7 \\
2.01 & $-27.75$ & $-7.15$ & 5.86 & 1 & 2.03 & 147 & 155.0 \\
2.01 & $-27.45$ & $-6.87$ & 8.03 & 1 & 2.02 & 276 & 291.0 \\
2.01 & $-27.15$ & $-6.67$ & 10.22 & 1 & 2.01 & 447 & 471.1 \\
2.01 & $-26.85$ & $-6.45$ & 13.97 & 0 & 1.99 & 648 & 682.7 \\
2.01 & $-26.55$ & $-6.24$ & 40.12 & 0 & 1.90 & 430 & 464.3 \\
2.01 & $-26.25$ & $-6.03$ & 495.10 & 0 & 1.87 & 30 & 39.4 \\
2.40 & $-28.95$ & $-8.12$ & 2.07 & 1 & 2.44 & 14 & 17.9 \\
2.40 & $-28.65$ & $-8.03$ & 2.30 & 1 & 2.41 & 17 & 21.8 \\
2.40 & $-28.35$ & $-7.59$ & 3.71 & 1 & 2.37 & 48 & 59.7 \\
2.40 & $-28.05$ & $-7.29$ & 5.28 & 1 & 2.37 & 98 & 121.2 \\
2.40 & $-27.75$ & $-7.05$ & 7.01 & 1 & 2.37 & 164 & 208.1 \\
2.40 & $-27.45$ & $-6.82$ & 9.50 & 0 & 2.38 & 265 & 356.0 \\
2.40 & $-27.15$ & $-6.61$ & 22.11 & 0 & 2.30 & 246 & 309.0 \\
2.40 & $-26.85$ & $-6.24$ & 249.51 & 0 & 2.25 & 37 & 48.8 \\
2.80 & $-29.55$ & $-8.57$ & 1.76 & 1 & 2.70 & 3 & 6.2 \\
2.80 & $-29.25$ & $-8.34$ & 1.84 & 1 & 2.82 & 7 & 10.6 \\
2.80 & $-28.95$ & $-8.08$ & 6.51 & 1 & 2.82 & 10 & 19.2 \\
2.80 & $-28.65$ & $-7.95$ & 3.68 & 1 & 2.80 & 12 & 25.9 \\
2.80 & $-28.35$ & $-7.65$ & 11.94 & 1 & 2.83 & 24 & 51.5 \\
2.80 & $-28.05$ & $-7.33$ & 15.75 & 1 & 2.81 & 50 & 107.9 \\
2.80 & $-27.75$ & $-7.11$ & 20.63 & 1 & 2.82 & 75 & 180.9 \\
2.80 & $-27.45$ & $-7.07$ & 24.17 & 1 & 2.79 & 73 & 199.8 \\
3.25 & $-29.55$ & $-8.54$ & 1.10 & 1 & 3.35 & 7 & 8.2 \\
3.25 & $-29.25$ & $-8.30$ & 1.45 & 1 & 3.25 & 12 & 14.2 \\
3.25 & $-28.95$ & $-8.33$ & 1.40 & 1 & 3.20 & 11 & 13.1 \\
3.25 & $-28.65$ & $-7.94$ & 2.18 & 1 & 3.25 & 28 & 32.5 \\
3.25 & $-28.35$ & $-7.64$ & 3.12 & 1 & 3.23 & 54 & 64.6 \\
3.25 & $-28.05$ & $-7.47$ & 3.89 & 1 & 3.25 & 77 & 95.9 \\
3.25 & $-27.75$ & $-7.32$ & 4.72 & 1 & 3.24 & 103 & 134.3 \\
3.25 & $-27.45$ & $-7.09$ & 6.47 & 1 & 3.21 & 161 & 228.8 \\
3.25 & $-27.15$ & $-6.99$ & 7.48 & 1 & 3.22 & 191 & 287.9 \\
3.25 & $-26.85$ & $-6.80$ & 10.40 & 0 & 3.20 & 234 & 377.5 \\
3.25 & $-26.55$ & $-6.63$ & 39.58 & 0 & 3.11 & 52 & 103.7 \\
3.75 & $-28.95$ & $-8.24$ & 1.56 & 1 & 3.69 & 14 & 15.7 \\
3.75 & $-28.65$ & $-8.02$ & 2.03 & 1 & 3.67 & 22 & 25.7 \\
3.75 & $-28.35$ & $-7.65$ & 3.06 & 1 & 3.77 & 54 & 60.5 \\
3.75 & $-28.05$ & $-7.64$ & 3.11 & 1 & 3.76 & 55 & 62.1 \\
3.75 & $-27.75$ & $-7.44$ & 4.07 & 1 & 3.74 & 83 & 99.3 \\
3.75 & $-27.45$ & $-7.27$ & 4.96 & 1 & 3.76 & 119 & 144.2 \\
3.75 & $-27.15$ & $-7.16$ & 6.59 & 0 & 3.72 & 117 & 158.4 \\
3.75 & $-26.85$ & $-6.89$ & 25.48 & 0 & 3.59 & 27 & 54.6 \\
4.25 & $-29.25$ & $-8.48$ & 1.16 & 1 & 4.25 & 8 & 8.4 \\
4.25 & $-28.65$ & $-8.18$ & 1.64 & 1 & 4.22 & 16 & 16.9 \\
4.25 & $-28.35$ & $-8.11$ & 1.79 & 1 & 4.19 & 19 & 20.0 \\
4.25 & $-28.05$ & $-7.91$ & 2.26 & 1 & 4.21 & 30 & 31.8 \\
4.25 & $-27.75$ & $-7.81$ & 2.53 & 1 & 4.24 & 38 & 40.2 \\
4.25 & $-27.45$ & $-7.59$ & 3.84 & 0 & 4.16 & 44 & 47.1 \\
4.75 & $-28.65$ & $-8.52$ & 1.14 & 1 & 4.66 & 7 & 7.4 \\
4.75 & $-28.35$ & $-8.46$ & 1.22 & 1 & 4.71 & 8 & 8.4 \\
4.75 & $-28.05$ & $-8.00$ & 2.07 & 1 & 4.66 & 23 & 24.2 \\
4.75 & $-27.75$ & $-8.06$ & 1.94 & 0 & 4.66 & 20 & 21.1 \\
4.75 & $-27.45$ & $-7.78$ & 20.57 & 0 & 4.62 & 6 & 8.3 \\

